OST: Efficient One-stream Network for 3D Single Object Tracking in Point Clouds

Although recent Siamese network-based trackers have achieved impressive perceptual accuracy for single object tracking in LiDAR point clouds, they usually utilized heavy correlation operations to capture category-level characteristics only, and overlook the inherent merit of arbitrariness in contrast to multiple object tracking. In this work, we propose a radically novel one-stream network with the strength of the instance-level encoding, which avoids the correlation operations occurring in previous Siamese network, thus considerably reducing the computational effort. In particular, the proposed method mainly consists of a Template-aware Transformer Module (TTM) and a Multi-scale Feature Aggregation (MFA) module capable of fusing spatial and semantic information. The TTM stitches the specified template and the search region together and leverages an attention mechanism to establish the information flow, breaking the previous pattern of independent \textit{extraction-and-correlation}. As a result, this module makes it possible to directly generate template-aware features that are suitable for the arbitrary and continuously changing nature of the target, enabling the model to deal with unseen categories. In addition, the MFA is proposed to make spatial and semantic information complementary to each other, which is characterized by reverse directional feature propagation that aggregates information from shallow to deep layers. Extensive experiments on KITTI and nuScenes demonstrate that our method has achieved considerable performance not only for class-specific tracking but also for class-agnostic tracking with less computation and higher efficiency.

==> relationship.tex <==
\section{Analysis of Our General Loss} \label{sec: relation}
In this paper, we set $\mathcal{H}(v_{tj}^p)$ as two different functions and deeply analyze two resulting losses. Besides, we find that logistic and triplet losses adopt in Siamese tracking network are particular cases of our informative enhanced loss under particular parameter settings. That is, as for Siamese network for visual tracking, the proposed loss is the root form of logistic loss \cite{Bertinetto2016SiamFC} and triplet loss \cite{Dong2018SiamFC-tri}, which brings a novel insight and could help us to re-understand the training process from a new perspective.
\subsection{Relation with the Logistic Loss}%Formula Manipulation of Logistic Loss
Let $\mathcal{H}(v_{tj}^p)=\log (1+e^{-v_{tj}^p})$, we can get the following inequalities based on the basic inequality $\log(\sum_i a_i)<\log (\prod_i (1+a_i))$ $(a>0)$,
\begin{small}
\begin{equation}\label{tau_1}
\begin{aligned}
  \tau_{tj}&=\max \left\{\max \limits_{(t,k) \in \mathcal{S}_n} (v_{tk}^n-\alpha),\max \limits_{(j,l) \in \mathcal{S}_n} (v_{jl}^n-\alpha)\right\}\\ & \quad+\log(1+e^{-v_{tj}^p})\\
  &\leqslant \log\left(\sum \limits_{(t,k) \in \mathcal{S}_n} e^{v_{tk}^n-\alpha}+\sum \limits_{(j,l) \in \mathcal{S}_n} e^{v_{jl}^n-\alpha}\right)\\ & \quad+\log(1+e^{-v_{tj}^p})\\
  &\leqslant \log\left(\prod \limits_{(t,k) \in \mathcal{S}_n} (1+e^{v_{tk}^n-\alpha}) \cdot \prod \limits_{(j,l) \in \mathcal{S}_n} (1+e^{v_{jl}^n-\alpha})\right)\\ &\quad+\log(1+e^{-v_{tj}^p}).
\end{aligned}
\end{equation}
\end{small}

In this paper, we introduce two parameters so as to enable a flexible control for two types of negative sample pairs. Afterwards, by replacing $\tau_{tj}$ in Eq.~(\ref{siamfc_iel_2}) with the last formula, we obtain our first surrogate loss function,
\begin{equation}\label{siamfc_iel_3}
  \tilde {L}_e=\frac{1}{2M}\sum_{(t,j) \in \mathcal{S}_p} {\hat\tau_{tj}},
\end{equation}
\begin{small}
\begin{equation}\label{siamfc_iel_tau_hat}
\begin{aligned}
  \hat\tau_{tj}&=\log(\prod \limits_{(t,k) \in \mathcal{S}_n} (1+e^{v_{tk}^n-\alpha})^{\lambda_1} \cdot \prod \limits_{(j,l) \in \mathcal{S}_n} (1+e^{v_{jl}^n-\alpha})^{\lambda_2})\\ &\quad+\log(1+e^{-v_{tj}^p}),
\end{aligned}
\end{equation}
\end{small}
where $\lambda_1$ and $\lambda_2$ are control factors. In particular, we can derive the logistic loss by setting $\lambda_1=\frac1N$, $\lambda_2=0$, and $\alpha=0$ in Eq. (\ref{siamfc_iel_tau_hat}).

\begin{algorithm}[t]
\caption{Backpropagation gradient}
\label{alg1}
\LinesNumbered
\KwIn{$v_{tk}^n, v_{tj}^p, v_{jl}^n, t\in\{1\}, j\in\{1, \cdots, M\}$, $k,l\in\{1,\cdots, N\}$}
\KwOut{$\frac{\partial \tilde {L}_e}{\partial \phi(z)}$, $\frac{\partial \tilde {L}_e}{\partial \phi(x_j)}$, $\frac{\partial \tilde {L}_e}{\partial \phi(x_i)}$, $j\in\{1, \cdots, M\}$, $i\in\{1, \cdots, N\}$}
$\frac{\partial \tilde {L}_e}{\partial \phi(z)}=0, \frac{\partial \tilde {L}_e}{\partial \phi(x_j)}=0, \frac{\partial \tilde {L}_e}{\partial \phi(x_i)}=0$\\
\For{$j=1, \cdots, M$}{
    \eIf{optimize Eq.(\ref{siamfc_iel_3})}{
        $\frac{\partial \tilde {L}_e}{\partial v_{tj}^p}=-\frac{1}{2M(1+e^{v_{tj}^p})}$\\%%
        $\frac{\partial \tilde {L}_e}{\partial \phi(z)}=\frac{\partial \tilde {L}_e}{\partial \phi(z)} + \frac{\partial \tilde {L}_e}{\partial v_{tj}^p} \frac{\partial v_{tj}^p}{\partial \phi(z)}$\\
        \For{$i, l, k=1, \cdots, N$}
        {$\frac{\partial \tilde {L}_e}{\partial v_{tk}^n}=\frac{\lambda_1}{2M(e^{-v_{tk}^n+\alpha}+1)}$\\
         $\frac{\partial \tilde {L}_e}{\partial v_{jl}^n}=\frac{\lambda_2}{2M(e^{-v_{jl}^n+\alpha}+1)}$\\%%
         $\frac{\partial \tilde {L}_e}{\partial \phi(z)}=\frac{\partial \tilde {L}_e}{\partial \phi(z)}+\frac{\partial \tilde {L}_e}{\partial v_{tk}^n} \frac{\partial v_{tk}^n}{\partial \phi(z)}$\\
         $\frac{\partial \tilde {L}_e}{\partial \phi(x_j)}=\frac{\partial \tilde {L}_e}{\partial \phi(x_j)}+\frac{\partial \tilde {L}_e}{\partial v_{jl}^n} \frac{\partial v_{jl}^n}{\partial \phi(x_j)} + \frac{\partial \tilde {L}_e}{\partial v_{tj}^p} \frac{\partial v_{tj}^p}{\partial \phi(x_j)}$\\
         $\frac{\partial \tilde {L}_e}{\partial \phi(x_i)}=\frac{\partial \tilde {L}_e}{\partial \phi(x_i)}+\frac{\partial \tilde {L}_e}{\partial v_{jl}^n} \frac{\partial v_{jl}^n}{\partial \phi(x_i)} + \frac{\partial \tilde {L}_e}{\partial v_{tk}^n} \frac{\partial v_{tk}^n}{\partial \phi(x_i)}$\\
        }}
        {
        // \emph{optimize Eq.(\ref{siamfc_iel_4})}\\
        \For{$i, l, k=1, \cdots, N$}
        {$\frac{\partial \tilde {L}_e}{\partial v_{tk}^n}=\frac{\lambda_1}{2M(e^{v_{tj}^p-v_{tk}^n+\alpha}+1)}$\\%
         $\frac{\partial \tilde {L}_e}{\partial v_{jl}^n}=\frac{\lambda_2}{2M(e^{v_{tj}^p-v_{jl}^n+\alpha}+1)}$\\%
         $\frac{\partial \tilde {L}_e}{\partial v_{tj}^p}= -\frac{\lambda_1}{2M(e^{v_{tj}^p-v_{tk}^n+\alpha}+1)}
         -\frac{\lambda_2}{2M(e^{v_{tj}^p-v_{jl}^n+\alpha}+1)}$\\
         $\frac{\partial \tilde {L}_e}{\partial \phi(z)}=\frac{\partial \tilde {L}_e}{\partial \phi(z)}+\frac{\partial \tilde {L}_e}{\partial v_{tk}^n} \frac{\partial v_{tk}^n}{\partial \phi(z)} + \frac{\partial \tilde {L}_e}{\partial v_{tj}^p} \frac{\partial v_{tj}^p}{\partial \phi(z)}$\\
         $\frac{\partial \tilde {L}_e}{\partial \phi(x_j)}=\frac{\partial \tilde {L}_e}{\partial \phi(x_j)}+\frac{\partial \tilde {L}_e}{\partial v_{jl}^n} \frac{\partial v_{jl}^n}{\partial \phi(x_j)} + \frac{\partial \tilde {L}_e}{\partial v_{tj}^p} \frac{\partial v_{tj}^p}{\partial \phi(x_j)}$\\
         $\frac{\partial \tilde {L}_e}{\partial \phi(x_i)}=\frac{\partial \tilde {L}_e}{\partial \phi(x_i)}+\frac{\partial \tilde {L}_e}{\partial v_{jl}^n} \frac{\partial v_{jl}^n}{\partial \phi(x_i)} + \frac{\partial \tilde {L}_e}{\partial v_{tk}^n} \frac{\partial v_{tk}^n}{\partial \phi(x_i)}$\\
        }
    }
}
\textbf{Return} $\frac{\partial \tilde {L}_e}{\partial \phi(z)}$, $\frac{\partial \tilde {L}_e}{\partial \phi(x_j)}$, $\frac{\partial \tilde {L}_e}{\partial \phi(x_i)}$
\end{algorithm}
\subsection{Relation with the Triplet Loss} %Formula Manipulation of Triplet Loss
Analogously, let $\mathcal{H}(v_{tj}^p)=-v_{tj}^p$, we obtain the following inequalities,
\begin{small}
\begin{equation}\label{tau_2}
\begin{aligned}
  \tau_{tj}&=\max \left\{\max \limits_{(t,k) \in \mathcal{S}_n} (v_{tk}^n-\alpha),\max \limits_{(j,l) \in \mathcal{S}_n} (v_{jl}^n-\alpha)\right\}-v_{tj}^p\\
  &\leqslant \log\left(\sum \limits_{(t,k) \in \mathcal{S}_n} e^{v_{tk}^n-\alpha}+\sum \limits_{(j,l) \in \mathcal{S}_n} e^{v_{jl}^n-\alpha}\right)-v_{tj}^p\\
  &= \log\left(\sum \limits_{(t,k) \in \mathcal{S}_n} e^{v_{tk}^n-v_{tj}^p-\alpha}+\sum \limits_{(j,l) \in \mathcal{S}_n} e^{v_{jl}^n-v_{tj}^p-\alpha}\right)\\
  &\leqslant \log\left(\prod \limits_{(t,k) \in \mathcal{S}_n} (1+e^{v_{tk}^n-v_{tj}^p-\alpha}) \cdot \prod \limits_{(j,l) \in \mathcal{S}_n} (1+e^{v_{jl}^n-v_{tj}^p-\alpha})\right).
\end{aligned}
\end{equation}
\end{small}

Based on the last inequality, we have another surrogate loss function,
\begin{equation}\label{siamfc_iel_4}
  \tilde{L}_e=\frac{1}{2M}\sum_{(t,j) \in \mathcal{S}_p} {\tilde\tau_{tj}},
\end{equation}
\begin{small}
\begin{equation}\label{siamfc_iel_tau_hat2}
  \tilde\tau_{tj}=\log(\prod \limits_{(t,k) \in \mathcal{S}_n} (1+e^{v_{tk}^n-v_{tj}^p-\alpha})^{\lambda_1} \cdot \prod \limits_{(j,l) \in \mathcal{S}_n} (1+e^{v_{jl}^n-v_{tj}^p-\alpha})^{\lambda_2}),
\end{equation}
\end{small}
where $\lambda_1$ and $\lambda_2$ are control factors. Note that, Eq. (\ref{siamfc_iel_tau_hat2}) becomes the triplet loss when $\lambda_1=\frac2N$, $\lambda_2=0$, and $\alpha=0$. 

Furthermore, by observing the above Eq. (\ref{siamfc_iel_tau_hat}) and Eq. (\ref{siamfc_iel_tau_hat2}), the derived surrogate loss consider not only the relationship of exemplar-positive pair $(t, k)$, but also the relationship of positive-negative pair $(j,l)$. This facilitates the network to balance similarities holistically. In detail, the gradients of Eq.~(\ref{siamfc_iel_3}) and Eq.~(\ref{siamfc_iel_4}) with respect to the input feature embeddings $\phi(z)$, $\phi(x_j)$, and $\phi(x_i)$ can be calculated according to Algorithm \ref{alg1}.





==> review.tex <==
\section{Review Losses of Two Siamese Trackers}
In this section, we briefly review the logistic loss and triplet loss of two fully convolutional Siamese networks, \ie, SiamFC~\cite{Bertinetto2016SiamFC} and SiamFC-tri\cite{Dong2018SiamFC-tri}.

\textbf{Siamese Network with Logistic Loss.}
In the searching image, a candidate patch refers to an instance $x$, which is generated by sliding window with the same size as the exemplar $z$. Specially, an instance is labeled as negative when its distance to the central location is larger than a threshold, otherwise is marked as positive. SiamFC~\cite{Bertinetto2016SiamFC} learns a similarity function $\Phi(z,x)$, which outputs a high score when two images are very similar, otherwise a low score. Similarity learning problem is modeled by a parameter sharing Siamese network, which can be viewed as an identical mapping $\phi$ for both the exemplar $z$ and instance $x$. After acquiring two representations $\phi(z)$ and $\phi(x)$, SiamFC adopts the cross correlation layer to compute the similarity. The formulation of $\Phi$ can be written as,
\begin{equation}\label{simafc_fun}
  \Phi(z,x)=\phi(z)*\phi(x)+b.
\end{equation}

Based on the above similarity function $\Phi(z,x)$ between the exemplar $z$ and instances $x$, SiamFC defines its logistic loss function as follows,
\begin{equation}\label{siamfc_loss}
  L_l=\frac{1}{2M} \sum_{i=1}^M {\log(1+e^{-v_i^p})}+\frac{1}{2N}\sum_{j=1}^N {\log(1+e^{v_j^n})},
\end{equation}
where $M$ is the number of positive instances, $N$ is the number of negative instances, $v_i^p$ is the response value generated by cross-correlating $i$-th positive instance with the exemplar, and $v_j^n$ is the response value generated by cross-correlating $j$-th negative instance with the exemplar.

\textbf{Siamese Network with Triplet Loss.}
In order to make full use of the input pairs of frames, SiamFC-tri\cite{Dong2018SiamFC-tri} constructs triplet connections among the exemplar, one positive instance, and one negative instances. Afterwards, it utilizes matching probability to calculate the local similarities in each triplet. Concretely, this method controls the response values $v_i^p$ and $v_j^n$ resorting to the softmax function,
\begin{equation}\label{siamfc_triplet_prob}
  prob(v_i^p, v_j^n)=e^{v_i^p}/(e^{v_i^p}+e^{v_j^n}).
\end{equation}
 
The triplet loss of SiamFC-tri aims to maximize the sum of the matching probabilities $\{prob(v_i^p, v_j^n)\}_{i=1,j=1}^{M,N}$ calculated in each triplet. After simple transformation, it can be eventually simplified as,
\begin{equation}\label{siamfc_triplet}
  L_t=\frac{1}{MN}\sum_{i=1}^M \sum_{j=1}^N {\log(1+e^{v_j^n-v_i^p})}.
\end{equation}
